Tunable RF-photonic filtering with high out-of-band rejection in silicon

The ever-increasing demand for high speed and large bandwidth has made photonic systems a leading candidate for the next generation of telecommunication and radar technologies. The photonic platform enables high performance while maintaining a small footprint and provides a natural interface with fiber optics for signal transmission. However, producing sharp, narrow-band filters that are competitive with RF components has remained challenging. In this paper, we demonstrate all-silicon RF-photonic multi-pole filters with $\sim100\times$ higher spectral resolution than previously possible in silicon photonics. This enhanced performance is achieved utilizing engineered Brillouin interactions to access long-lived phonons, greatly extending the available coherence times in silicon. This Brillouin-based optomechanical system enables ultra-narrow (3.5 MHz) multi-pole response that can be tuned over a wide ($\sim10$ GHz) spectral band. We accomplish this in an all-silicon optomechanical waveguide system, using CMOS compatible fabrication techniques. In addition to bringing greatly enhanced performance to silicon photonics, we demonstrate reliability and robustness, necessary to transition silicon-based optomechanical technologies from the scientific bench-top to high-impact field-deployable technologies.

==> figures/LNA.tex <==
\begin{figure*}[hb!]
    \centering
    \includegraphics[scale=0.8]{figures_graphics/LNA_new-eps-converted-to.pdf}
    \caption{
    a. Measurements of a single tone, 10 MHz from the filter center-frequency, with (red) and without (blue) an RF amplifier at the link input. The thermal-Brillouin noise can be seen around the center of the pass-band. The bandwidth used in the measurements was 51 kHz.
    b. Magnified view of the Brillouin noise (gray boxed region in panel a.) showing the noise floor does not change with the input RF power, nor with the addition of the RF amplifier.
    c. Magnified view of the signal after passing through the PPER filter (green boxed region in panel a.) showing higher output RF power with the addition of the amplifier.
    \ref{tbl:RF_table}.}
    \label{fig:LNA}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
